Usable & Scalable Learning Over Relational Data With Automatic Language Bias

Relational databases are valuable resources for learning novel and interesting relations and concepts. In order to constraint the search through the large space of candidate definitions, users must tune the algorithm by specifying a language bias. Unfortunately, specifying the language bias is done via trial and error and is guided by the expert's intuitions. We propose AutoBias, a system that leverages information in the schema and content of the database to automatically induce the language bias used by popular relational learning systems. We show that AutoBias delivers the same accuracy as using manually-written language bias by imposing only a slight overhead on the running time of the learning algorithm.

==> 6.Experiments-Sampling.tex <==
\subsection{Evaluating Sampling Techniques}
\label{section:automode-experiments-sampling}

In this section, we empirically evaluate the sampling techniques presented in Section~\ref{section:automode-sampling}.
We use three versions of Castor. Each version uses a different sampling technique for bottom-clause construction:
\begin{enumerate}
	\item {\bf Castor-Na\"ive} uses na\"ive sampling, as explained in Section~\ref{section:automode-naive-sampling}. 
	\item {\bf Castor-Random} uses random sampling, as explained in Section~\ref{section:automode-random-sampling}. Random sampling is implemented using Olken's sampling approach.
	\item {\bf Castor-Stratified} uses stratified sampling, as explained in Section~\ref{section:automode-stratified-sampling}. 
\end{enumerate}

We use two different methods for setting the language bias: manual tuning and AutoMode.
Table~\ref{table:automode-sampling-results} shows the results of Castor learning over the HIV dataset with different sampling techniques and using different methods for setting the language bias.
Using both manual tuning and AutoMode, Castor-Stratified obtains the best recall and a competitive precision.
Castor-Random obtains a better precision and recall than Castor-Na\"ive and is the most efficient.
Castor-Na\"ive obtains the lowest precision and recall.
In the HIV database, compounds contain hundreds of atoms. Some atoms are common elements, e.g., Hydrogen, while other atoms are rare elements, e.g., Lithium.
Castor-Stratified is able to explore join paths that lead to all types of elements in a compound.
Therefore, the bottom-clauses generated by Castor-Stratified contain diverse information, which allows it to learn better definitions.
Castor-Random focuses on obtaining a subset of the data that is representative of the whole data, but is not necessarily helpful for learning definitions.
Castor-Na\"ive simply samples tuples uniformly in each relation.

In general, the best sampling technique is the one that allows Castor to run efficiently and learn effective definitions.
The efficiency is affected not only by the time taken to build a bottom-clause, but also by the speed in which effective definitions are discovered.
Castor uses the covering approach (Algorithm~\ref{algorithm:castor-covering}).
Each time that a learned clause satisfies the minimum criterion, it is added to the definition and all positive examples covered by the clause are removed. 
If clauses that cover many positive examples are discovered early, then less positive examples must be used to generate candidate definitions. Therefore, the learning process is more efficient.
Castor-Stratified provides the best trade-off between effectiveness of the learned definitions and learning time.


\begin{table*}
	\centering
	\caption{Results of learning relations over HIV data with different sampling techniques (m=minutes).}
	\begin{tabular} { c | c c c | c c c}
		\hline
		\multirow{2}{*}{Measure} & \multicolumn{3}{c|}{Manual tuning} & \multicolumn{3}{c}{AutoMode} \\
		\cline{2-7}
		 & Castor-Na\"ive  & Castor-Random & Castor-Stratified & Castor-Na\"ive  & Castor-Random & Castor-Stratified \\
		\hline
		Precision & 0.74 & 0.83 & 0.81 & 0.80 & 0.83 & 0.81 \\
		Recall & 0.84 & 0.86 & 0.91 & 0.85 & 0.86 & 0.92\\
		Time & 22.6m & 20.2m & 24.3m  & 35.1m & 19.9m  & 25m\\
	\end{tabular}
	\label{table:automode-sampling-results}
\end{table*}

%\begin{table}
%	\centering
%	\caption{Results of learning relations over HIV data with different sampling techniques (h=hours, m=minutes).}
%	\begin{tabular} { c c c c c }
%		\hline
%		\multirow{2}{*}{Dataset} & \multirow{2}{*}{Measure} &  Castor-  & Castor- & Castor- \\
%		& & Na\"ive &  Random & Stratified \\
%		\hline
%		\multirow{3}{*}{HIV-Large}  & Precision & 0.80 & 0.84 & 0.87 \\
%		& Recall & 0.77 & 0.73 & 0.88 \\
%		& Time & 7.4h & 6.3h  & 6.1h  \\
%		\hline
%		\multirow{3}{*}{HIV-2K4K}  & Precision & 0.74 & 0.83 & 0.81 \\
%		& Recall & 0.84 & 0.86 & 0.91 \\
%		& Time & 22.3m & 20.2m & 24.3m  \\
%	\end{tabular}
%	\label{table:automode-sampling-results}
%\end{table}
